A Review of Surface Haptics:Enabling Tactile Effects on Touch Surfaces

We review the current technology underlying surface haptics that converts passive touch surfaces to active ones (machine haptics), our perception of tactile stimuli displayed through active touch surfaces (human haptics), their potential applications (human-machine interaction), and finally the challenges ahead of us in making them available through commercial systems. This review primarily covers the tactile interactions of human fingers or hands with surface-haptics displays by focusing on the three most popular actuation methods: vibrotactile, electrostatic, and ultrasonic.

==> SChoi/Intro-humanhaptics.tex <==
%\subsection{Human haptics}



==> old_sections/introduction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}

\IEEEPARstart{H}{aptics} for interactive touch surfaces, also known as surface haptics, is a new area of research in the field of haptics. The goal of surface haptics is to generate tactile effects on touch surfaces such as those used in mobile phones, tablets, kiosks and information displays, and front panels of new generation home appliances and cars.

Integration of haptics into touch surfaces will result in new applications in user interface design, online shopping, gaming and entertainment, education, arts, and more. Imagine that you feel the fabric of a blue-jean that you purchase from internet on your tablet, or the edges of dial buttons on your mobile phone so that you can dial a number even without looking at the screen (as in earlier generation mobile phones), that you can play chess against a computer on an interactive touch surface and feel a frictional resistance when you make an incorrect move, and that you can feel the detents of a digital knob displayed on the touch surface of your car or oven as you rotate it, that a visually impaired person utilizes a haptic map displayed on a tablet for navigation in a building, or your children feels the skin of an exotic animal on an interactive touchscreen used in a classroom.

As obvious from the examples above, surface haptics is a new and exciting area of research and the number of potential applications of this technology is countless. Moreover, we anticipate that surface haptics in the future will not be restricted to touch surfaces of electronic devices only but will be available in any flat or curved physical surface made of hard or soft material and having some form of embedded computational capability.

This review primarily covers the tactile interactions of human finger/hand with surface-haptics displays by focusing on the three most popular actuation methods: vibrotactile, electrostatic, and ultrasonic. We intentionally excluded some other less-common actuation methods such as electromagnetic actuation (e.g., \cite{Jansen10}) and methods utilizing fluidic pressure \cite{Craig12} as well as kinesthetic haptic interactions (not primarily involves tactile channel) with shape-changing surfaces (e.g., \cite{Follmer13}), indirect haptic interactions with touch surfaces such as mid-air haptics via acoustic radiation pressure (e.g., \cite{Hoshi10}) and through hand-held devices such as pen/stylus from our review (e.g., \cite{Kyung09}).

We review the current state of the art in terms of 1) machine haptics: technologies to generate tactile stimuli on touch surfaces and the physics behind it, 2) human haptics: our tactile perception of those stimuli, 3) human-machine haptics: interactions between those two, leading to rendering of virtual shapes, textures, and controllers with potential applications in the areas discussed above.

%\hl{Missing an overview of the structure of the paper and the subsections of the Introduction.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Machine haptics}

Here, we provide a basic introduction of the current technologies enabling tactile feedback on touch surfaces. We first group them based on the direction of stimulation and then briefly discuss how each technology works. More details on the earlier studies are available in the literature review section (Section 2). 

From the technological point of view, the goal of surface haptics is to design and develop new devices in order to display tactile feedback to the users by modulating the interaction forces between the finger and the touch surface. In this regard, the current technologies can be grouped based on the direction that the finger is stimulated by the interaction forces (see Fig. 1): a) normal to the surface, b) tangential to the surface, and c) both.  


%The first requirement is that the tactile feedback should not change the functionality of the surface. For instance, if this surface lies on top of a display, it should remain transparent. Also, user’s fingertips moves freely on the surface, and by principle, no actuator should be attached to the fingertip to produce the stimulation. Having this in mind, and apart of some exotic examples~\cite{Craig12}, it has been easier on a technological point of view not to change to geometry of the surface, but instead, to modulate the contact forces between the surface and the fingertip. To achieve such a goal, the examples proposed in the literature review can be shared into two principles: forces generated normal to the surface, or instead parallel to it.
%

\begin{figure}[ht]
\centering
\includegraphics[width=1.0\columnwidth]{img/normal_vs_tangential.png}
\caption{Basic principle of contact force modulation in a haptic surface}
\label{fig:normal_vs_tangential}
\end{figure}

\begin{figure*}[hbt]
    \begin{center}
        %\includegraphics[width=0.9\textwidth]{img/Table_Technology.png}
        \input{img/figure_2.tex}
    \end{center}
\caption{Classification of the current technologies for haptic surfaces.}
\label{fig-clas_Fig}
\end{figure*}

When the stimulation is in the normal direction, an actuator placed in the periphery of the surface creates a mechanical vibration that propagates inside the material and reaches the finger pulp~\cite{Poupyrev:2002, Yao:2010}. This type of stimulation is referred to as vibrotactile, because the vibrations are directly detectable by our tactile system ($<$1kHz). In fact, vibration motors are already embedded in mobile phones today and utilized to alert the user about incoming calls and also to provide confirmation for button press events. Although it is highly difficult to generate complex tactile effects using these simple motors, they have been preferred by the manufacturers over voice coils and piezo actuators due to their low-cost and low energy requirements.

Using more advanced actuators and techniques, localizing the vibrations within a specific area of the tactile surface is possible. For that purpose, several actuators are placed on the surface, and their control signals are synchronized in order to obtain constructive and destructive waves where needed. The theory behind this principle has been investigated under the names of \textit{inverse filtering}~\cite{Hudin:2018}, \textit{modal composition}~\cite{Woo:2015, Enferad:2018} and \textit{time reversal}~\cite{Bai:2011, Hudin:2013}.

It is also possible to stimulate the finger in tangential direction for displaying tactile effects if there is a relative motion between the finger and tactile surface. For example, due to the viscoelastic properties of the finger pulp, the lateral movement of the tactile surface can induce tangential forces inside the finger pulp. By modulating this lateral movement as a function of the finger displacement, it is even possible to render virtual textures on a tactile surface~\cite{wiertlewski:2011}. Indeed, by means of a phenomenon called \textit{causality inversion}, the forces produced by the lateral movement of the tactile surface can be matched to those produced by a real textured surface when a finger slides on it. 

Alternatively, researchers have devised ways to dynamically change the friction forces between the tactile surface and the finger siding on its surface. This can be, for example, achieved by using actuators that generate micro-scale vibrations on the tactile surface at ultrasonic frequencies~\cite{Nara:2001, Biet:2007, Winfield:2007, ghenna:2017}. The vibration reduces the friction coefficient, a phenomenon called \textit{active lubrication}, because the finger is in intermittent contact with the plate. Using this approach, it is possible to simply turn the actuation on and off to generate relatively simple tactile effects in open-loop or to control the amplitude of vibrations in closed-loop to generate more complex tactile effects.

Instead of decreasing the friction via ultrasonic actuation, it is possible to increase it by using electrostatic actuation. This involves applying a voltage to the conductive layer of a tactile surface to generate electrostatic attractive forces in the normal direction between its surface and a finger sliding on it, which leads to an increase in frictional forces applied to the finger opposite to the direction of movement. Although the magnitude of this electrostatic force in normal direction is small relative to the normal load applied by the finger, it results in a perceivable frictional force in tangential direction when the finger slides on the touch screen. This frictional force can be modulated to generate different tactile effects by altering the amplitude, frequency and phase of the voltage signal applied to the touch surface.

In order to modulate the tangential forces on the plane of tactile surface to obtain a net force (i.e. vectorial summation of tangential forces), one can move the tactile surface in the direction tangent to the finger movement on the  same plane while modulating the friction using either ultrasonic or electrostatic actuation. This technique, named \textit{shivering} can produce net forces with very low lateral displacements of the surface. Finally, by combining bending modes at high frequency of the surface, it is also possible to produce such a net force, by using elliptical movement of the surface’s particles.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Section 1.2. Human Haptics
\input{SChoi/Intro-humanhaptics.tex}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Human-Machine Haptics}

Lead: VL

\begin{itemize}
\item What are the potential HCI paradigms for surface haptics?
\item Interaction types:
    \begin{itemize}
    \item static (e.g.vibrotactile) versus dynamic (e.g. friction modulation by electrovibration/ultrasonic)
    \item single vs multi-finger tactile
    \end{itemize}
\item What can be rendered on touch surfaces?
    \begin{itemize}
    \item shapes, textures, virtual controls (detents, buttons, knobs, etc).
    \end{itemize}
\item How do we design a haptic UI for touch surfaces? What is UIX and how does surface haptics is expected to enhance UIX?
\item User-centered design, sketching, prototyping
\end{itemize}

\hl{Vincent: This section should introduce the fundamentals, please keep more details for Section 2.}


==> old_sections/review.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Review of literature (9-11 pages)}

\hl{MISSING TABLE}

What is the current state of the art ?
\begin{itemize}
\item Vibrotactile: Lead: SC, Contributors: VL, FG, CB
           	ERM, LRA, Voice Coil Motors-bending wave haptics, Apple-Taptic Engine: iphone 7 , Piezoactuators
	\hl{Seungmoon: Proceedings of IEEE paper (nice review)}~\cite{Choi13}

\item Ultrasonic; Lead: FG, Contributors: CB,?
Piezoactuators: vertical/horizontal waves
 
\item Electrostatic; Lead: CB, Contributors: SC, FG, VL
Surface Capacitive vs Projected Capacitive?
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Machine haptics}

Studies on the design and evaluation of various actuation technologies (vibrotactile, electroadhesive, ultrasonic) for displaying haptic feedback through touch surfaces and the physics behind it.

\subsubsection{Vibrotactile Actuation}
% lead: SC + VL

\hl{Physics of Vibrotactile Actuation}
\hl{Propagation of vibration on the touch surface (normal vs tangential)}

While an electric motor is compact, cost effective, and easy to integrate into a touch screen, it operates in a narrow frequency range, limiting its bandwidth. To be able to use a wide range of actuation frequencies and hence to create richer haptic effects, piezo actuators are preferred over electric motors. The piezo actuators are also compact and can be easily mounted on a touch screen, but typically require higher voltage input. 

One of the challenges in vibrotactile actuation is to generate localized effects on touch surfaces. In~\cite{Dhiab:2019}, \hl{include size of the plate} the authors adjust the geometrical parameters (width, length, thickness and bounding conditions) of the surface in order to confine the vibration by an actuator at its exact location. This solution is robust besides the technology of actuator (piezoelectric or magnetic), but the actuator should be transparent so as not to obstruct the view. In \cite{Duong:2019}, the authors cover the entire surface with a relaxor ferroelectric polymer (RFP) transparent film, and produce vibrotactile stimulation based on the fretting phenomenon. They could create vibration at 500Hz, with an amplitude of 1$\mu m$ with a voltage amplitude of 200 V.

In Emgin et al.~\cite{Emgin19} the authors attached four piezoelectric patches to the edges of a touch screen to control out–of plane vibrations and display localized vibrotactile haptic feedback to the user. For this purpose, a vibration map of the touch surface was constructed in advance and then vibrotactile haptic feedback was displayed to the user using this map during real–time interaction. To construct the vibration map, the surface was divided into 84 grid points (7 rows by 12 columns) and the out–of–plane vibrations at each grid point were measured for the applied voltage when each piezo patch was excited individually and also when all patches were excited together. This process resulting in 5 frequency response functions (FRFs) for each grid point, one for individual piezo patches and one for all. In order to display localized vibrotactile haptic feedback on the touch surface, they utilized these five FRF functions of 84 grid points (referred to as “vibration map”). They achieved localized haptic feedback by maximizing the vibration at one grid point, while minimizing it at the others (note that for each grid point, there is an excitation frequency at which the amplitude is maximum. If the surface is excited at this frequency, a localized haptic effect can be generated at and around that point)\hl{some performances may be required here}.

These techniques however do not really focus the stimulation on a specific area. For that purpose, vibration modes of the plate can be composed to create a vibration pattern that is detectable by the fingertip. In \cite{Woo:2015}, 34 electromagnetic actuators located at the periphery of a $268 \times 170 \times 0.7 mm^3$ glass plate, could control 34 vibration modes, and create a pulse on a $50 \times 50 mm^2$ spot. To increase the contrast (the ratio of the vibration amplitude at the focus point to the vibration anywhere else on the plate), the time reversal technique can be used. In \cite{Bai:2011} for instance, the authors used 4 electromagnetic actuators to create a 3ms pulse on a $0.42\times 0.42\times 0.002 mm ^3$, with 1mm height on a spot 2cm in diameter. Higher contrast is obtained in \cite{Hudin:2015}; with 32 piezoelectric actuators, the authors could create a 7$\mu m$ pulse on a spot 5.2mm in diameter. The plate is $148 \times 210 \times 0.5 mm^3$. 

\subsubsection{Electrovibration}
% Lead: CB

The electrical attraction between human skin and a charged surface is not new and was first reported by Johnsen and Rahbek in 1923~\cite{Johnsen23}. Approximately thirty years later, Mallinckrodt discovered by accident that dragging a dry finger over a conductive surface covered with a thin insulating layer and in the presence of the alternating voltage can increase friction during touch~\cite{Mallinckrodt53}. He explained this phenomenon based on the well-known principle of parallel plate capacitor. Later, Grimnes named this phenomenon as electrovibration (electrically induced vibrations) and reported that surface roughness and dryness of finger skin could affect the perceived haptic effects~\cite{Grimnes83}. Afterwards, Strong and Troxel~\cite{Strong70} developed an electrotactile display consisting of an array of electrodes insulated with a thin layer of dielectric. Using friction induced by electrostatic attraction force, they generated texture sensations on the touch surface. Their experimental results showed that the intensity of touch sensation was primarily due to the applied voltage rather than the current density. Beebe et al. [10]~\cite{MISSING}, developed a polyimide-on-silicon electrostatic fingertip tactile display using lithographic microfabrication. They were able to generate tactile sensations on this thin and durable display using 200-600 V voltage pulses and reported the perception at the fingertip as “sticky.” Later, Tang and Beebe [11]~\cite{MISSING} performed experiments of detection threshold, line separation and pattern recognition with visually impaired subjects. Although they encountered problems such as dielectric breakdown and sensor degradation, the subjects were able to differentiate simple tactile patterns by haptic exploration. Agarwal et al. [12]~\cite{MISSING} investigated the effect of dielectric thickness on haptic perception during electrostatic stimulation. Their results showed that variations in dielectric thickness had little effect on the threshold voltage.

More recently, Bau et al.~\cite{Bau10} and Linjama et al. [2]~\cite{MISSING} have shown that electrovibration can be delivered through a commercial capacitive touch screen, which demonstrates the viability of this technology on mobile applications. A surface capacitive touchscreen consists of a glass substrate, coated with a conductive layer such as Indium Tin oxide (ITO), and an insulating layer such as Silicon dioxide (SiO2). When an alternating voltage is applied to its conductive layer, as the human body is also an electrical conductor, touching the surface of the screen results in an attraction force between finger and surface of touchscreen due to the induction of charges with opposite sign on the insulating layer of the glass substrate and the finger. 

While the technology for generating tactile feedback on a touch screen via electrovibration is already in place and straightforward to implement, our knowledge on the underlying contact mechanics and tactile perception are highly limited [10]~\cite{MISSING}. This is not surprising since the contact interactions between human skin and a counter surface is already highly complex to investigate even without electrovibration [11-13]~\cite{MISSING}. In the case of electrovibration in particular, the exact mechanism leading to an increase in tangential frictional forces is still not known completely. To estimate the electrostatic forces between finger pad and touch screen, models based on parallel-plate capacitor theory have been proposed (see the summary in Vodlak et al. [14]~\cite{MISSING}). These models assume a constant air gap between two surfaces and ignore the rounded shape of the finger pad and the asperities on its surface. On the other hand, to estimate the frictional forces in tangential direction during sliding, the Coulomb model of friction utilizing a constant coefficient of dynamic friction between finger pad and touch screen has been used so far. The increase in tangential force has been explained by simply adding the force due to electrostatic attraction to the normal force applied by the finger, $F_t=\mu(F_n+F_e)$, where $\mu$ is the friction coefficient, $F_t$, $F_n$, and $F_e$ represent the tangential, normal, and electrostatic forces, respectively. However, friction of human skin against smooth surfaces is governed by adhesion model of friction [15-17]~\cite{MISSING}, which depends on interfacial shear strength and real area of contact. The frictional force due to adhesion is given by , where $\tau$ is the interfacial shear strength and Ar is the real area of contact. It is highly difficult to measure or estimate the real area of contact, which varies nonlinearly with the normal force. In earlier studies, the real contact area has been taken as the contact area of finger ridges, $A_ridge$, which is smaller than the apparent contact area, Aapparent, estimated by the fingerprint images, using the boundaries of finger pad in contact with surface [18]~\cite{MISSING}. On the other hand, if the Persson’s contact theory is considered (also see the review of other contact theories in the same study [19]~\cite{MISSING}), the real area of contact ($A_r$) is, in fact, much smaller than the contact area of finger ridges (Aridge) since only the finger asperities at finer resolution make contacts with the surface. Recently, Persson (2018) extended his theory to electroadhesion and derived a mathematical relation for electroadhesive pressure between two conductive surfaces with random roughness in contact for voltage applied to one of the conducting surfaces. He assumed the small slope approximation ($|\nabla u| << 1$) for the roughness profiles and solved the Laplace equation for electrostatic potential to obtain the pressure due to electroadhesive force for the applied voltage. He used the normal pressure to estimate the real contact area and then the tangential friction force as Ft = Areal x Shear Stress. The application of this approach to the interactions between human finger and touch screen under electroadhesion has been investigated by Ayyildiz et al. (2018) and Sirin et al. (2019) and verified by the experimental data collected via custom-made tribometer. These studies show that electrostatic attraction force increases the real contact area between fingerpad and  touchscreen, leading to an increase in sliding friction force (Ayyildiz et al., 2018; Sirin et al., 2019a). The authors argue that the artificially generated electrostatic force results in a decrease in interfacial gap and hence the finger asperities make more contacts with the surface of the touch screen at the microscopic scale, leading to a decrease in an increase in real contact area of finger. Supporting this claim, Shultz et al. (2018) showed that the electrical impedance of the interfacial gap is significantly lower for the stationary finger compared to that of the sliding finger under electroadhesion. In contrast to the argument on increase in real contact area, which is highly difficult to measure and validate experimentally, the decrease in apparent contact area under electrovibration has been already demonstrated recently. Sirin et al. (2019b) conducted an experimental study to investigate the contact evolution between the human finger and a touch screen under electrovibration using a robotic set-up and an imaging system. The results show that the effect of electrovibration is only present during full slip but not before slip. Hence, the coefficient of friction increases under electrovibration as expected during full slip, but the apparent contact area is significantly smaller during full slip when compared to that of no electrovibration condition. It was suggested that the main cause of the increase in friction during full slip is due to an increase in the real contact area and the reduction in apparent area is due to stiffening of the finger skin in the tangential direction.

\subsubsection{Ultrasonic Actuation}

When a finger slides over a high frequency vibrating plate , the friction that produces this motion decreases as the vibration amplitude increases. This phenomenon, called \emph{active lubrication} has been first introduced by \cite{Watanabe95} to create a tactile stimulator. So far, two different mechanisms have been suggested to explain the cause of friction reduction in ultrasonic tactile displays;  \cite{Biet:2007} proposed that the friction reduction is due to the formation of a squeeze film of air between finger and the surface. Alternatively, it has been suggested that, when a surface vibrates at an ultrasonic frequency, an intermittent mechanical contact develops between finger and the surface such that the finger bounces on the surface while sliding~\cite{dai:2012,Vezzoli:2017}. A recent study conducted by Wiertlewski et al. \cite{Wiertlewski16} using a stroboscope revealed that both mechanisms indeed contribute to the friction reduction. Hence, it appears that the fingertip bounces on a cushion of squeezed film of air. Ultrasonic actuation can provide a higher variation in friction as compared to the electrostatic actuation, while the rendering bandwidth of ultrasonic devices is limited due to its resonating nature~\cite{Vardar17}.

To generate the vibration of the touched surface, piezoelectric cells are glued and supplied by sinusoidal voltages at a frequency above 20kHz. To efficiently produce this vibration, a stationary bending mode is energized, and specific design procedure is carried out in order to optimize the power efficiency \cite{giraud:2010, Wiertlewski15} and to free the screen of the tactile plate from non-transparent actuators \cite{giraud:2012}; for this last example, $400mW$ of power were needed at 150V peak to produce a vibration amplitude of $1.5\mu m$ peak at 31kHz on a $93 \times 65 \times 0.9 mm^3$ glass plate. Evidence for tactile stimulation at higher frequencies has been reported at 881kHz~\cite{takasaki:2019}.
The combination of two vibration modes is also possible at ultrasonic frequency. This can lead to dual-touch tactile stimulator, as in \cite{ghenna:2017} where two vibration modes are controlled in amplitude and phase in order to differentiate the vibration at two points of the plate.




%However, it is possible to implement electrostatic and ultrasonic actuation techniques together on the same surface to achieve even larger variation in friction coefficient [8]~\cite{MISSING}.

\hl{Frederic: More?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Human haptics}

This section covers the studies on surface haptics investigating human perception, cognition, attention, mechanics and neuroscience of contact between the human fingerpad and touch surfaces displaying haptic feedback.

\subsubsection{Tactile Perception by Vibrotactile}
\hl{SC}

Mechanics of Vibrotactile Stimulation:
\begin{itemize}
\item Impedance in normal and tangential direction
\item Propagation of vibration on the finger (Yon has done some work)
\item Effect of finger skin material properties on tactile feeling of vibrotactile stimulus
\item Neuroscience/Mechanotransduction aspects?
\end{itemize}

\subsubsection{Tactile Perception by Electrovibration}
\hl{CB}

The studies on tactile perception by electrovibration so far mainly focused on the estimation of perceptual thresholds for periodic stimuli. Bau et al. measured the sensory thresholds of electrovibration using sinusoidal inputs applied at different frequencies [6]~\cite{MISSING}. They showed that the change in threshold voltage as a function of frequency followed a U-shaped curve similar to the one observed in vibrotactile studies. Later, Wijekoon et al. [10]~\cite{MISSING}, followed the work of [23]~\cite{MISSING}, and investigated the perceived intensity of modulated friction generated by electrovibration. Their experimental results showed that the perceived intensity was logarithmically proportional to the amplitude of the applied voltage signal. Vardar et al. [8,24]~\cite{MISSING} investigated the effect of input voltage waveform on our tactile perception of electrovibration. Through psychophysical experiments with 8 subjects, they showed that humans were more sensitive to tactile stimuli generated by square wave voltage than sinusoidal one at frequencies below 60 Hz. In order to interpret the outcome of these experiments, the force and acceleration data collected from the subjects was analyzed in the frequency domain by taking into account the human vibrotactile sensitivity curve. This detailed analysis showed that Pacinian channel was the primary psychophysical channel in the detection of the electrovibration stimuli, which is most effective to tactile stimuli at high frequencies around 250 Hz. Hence, the stronger tactile sensation caused by a low-frequency square wave was due to its high- frequency components stimulating the Pacinian channel. Vardar et al. [25]~\cite{MISSING} investigated the interference of multiple tactile stimuli under electrovibration. Previous vibrotactile studies have already shown that presenting one stimulus may interfere with the perception of another one. This interference is called tactile masking and can cause certain deficits in perception such as increasing detection thresholds and hindering localization or identification. Considering the fact that the interaction area of touch screens is much larger than those used in earlier vibrotactile studies, tactile masking has a greater potential for digital applications utilizing electrovibration. They conducted psychophysical experiments and showed that masking effectiveness was larger with pedestal masking than simultaneous one. They also showed that sharpness perception of virtual edges displayed on touch screens depends on the "haptic contrast" between background and foreground stimuli, similar to the way it has been observed in vision studies, which varies as a function of masking amplitude and activation levels of frequency-dependent psychophysical channels. Later, Jamalzadeh et al. (2019)~\cite{MISSING} investigated whether it is possible to change the detection threshold of electrovibration at fingertip of index finger via remote masking, i.e. by applying a (mechanical) vibrotactile stimulus on the proximal phalanx of the same finger. The masking stimuli were generated by a voice coil (Haptuator). For eight participants, they first measured the detection thresholds for electrovibration at the fingertip and for vibrotactile stimuli at the proximal phalanx. Then, the vibrations on the skin were measured at four different locations on the index finger of subjects to investigate how the mechanical masking stimulus propagated as the masking level was varied. Finally, electrovibration thresholds were measured in the presence of vibrotactile masking stimuli. The results showed that vibrotactile masking stimuli generated sub-threshold vibrations around fingertip and, hence, did not mechanically interfere with the electrovibration stimulus. However, there was a clear psychophysical masking effect due to central neural processes. Electrovibration absolute threshold increased approximately 0.19 dB for each dB increase in the masking level. 

\subsubsection{Tactile Perception by Ultrasonic}
\hl{Frederic?}
Tactile perception of change in friction (discuss fundamentals here, how it is applied to rendering should go to section 2.3)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Human-Machine Haptics}

Touch-enabled devices like smart-phones and tablets are ubiquitous today, and are being used on a daily basis. All the devices commercially available today provide visual and auditory feedback to their users but almost no tactile feedback, though it is known that tactile feedback improves task performance and realism when interacting with digital data. Moreover, tactile sensation is a significant factor for preference and admiration of certain consumer products due to their texture. Therefore, a great deal of research is being carried out in recent years to develop and study the techniques that can render tactile information on touch-enabled devices.

\begin{itemize}
\item Tactile rendering algorithms for displaying virtual shapes and textures on touch surfaces
\item New HCI paradigms, and user interface design and experience (UIX)
\item Applications of surface haptics in consumer electronics, the automotive industry, home appliances, designing aids for the visually impaired, online shopping, gaming and entertainment, data visualization, education, and art appreciation
\end{itemize}

General introduction to touch surfaces:
need for multitouch, not limited to touchscreens, DIY, etc.

Sketching and prototyping?
\cite{Levesque11}

Multitouch:
tricks to make electrovibration work with multitouch \cite{Bau10}
electrode arrays to support multitouch (discuss in HW section, future challenges?)

Designing widgets and touch interactions to maximize sliding
\cite{Levesque11,Levesque12} + patents?

Target acquisition with friction displays:
\cite{Levesque11,Casiez11,Zhang15}

Affective communication:
~\cite{Mullenbach14}

Applications of programmable friction: 
\cite{Levesque11,Bau10}

Tactile rendering by electrovibration:
\cite{Kim13}

Feeling objects at a distance by electrovibration for the blind:
\cite{Israr12}

Tactile graphics by electrovibration:
\cite{Xu11}

Reverse electrovibration / AR, everyday objects
\cite{Bau12,Bau12a}

Scrolling interactions
\cite{Levesque12}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Tactile Rendering for Virtual Controls}
\hl{CB}

In contrast to physical controls, virtual controls displayed on tabletops cannot be felt. As a result, task precision and performance drop [2]~\cite{MISSING}. Moreover, lack of haptic feedback requires continuous visual attention on the controller. For example, graphical knobs with visual detents (notches) is frequently used in tabletop displays to rotate a virtual object in the scene or select an item from a menu using rotation gesture. Lack of haptic feedback makes it difficult for the user to precisely rotate the object or quickly select the item from the menu. Moreover, they cannot rest their fingers on the knob and focus on the virtual object or the menu. An alternative to virtual control is tangible control. In this approach, portable physical controls are directly placed on a tabletop to augment visual interfaces with haptic feedback. These controls are detected with the help of touch sensing overlays or cameras. For example, PhotoHelix is a physical knob placed on a tabletop to interact with digital photo collection [27]~\cite{MISSING}. In this approach, one hand rotates the physical knob to control position on a helix–shaped calendar while the other hand inspects and modifies the digital photos. The translucent tangible knob in SLAP widgets can be used in various modes to interact with digital content depending on the application [28]~\cite{MISSING}. For example, the knob can be used in the “jog wheel” mode to find and mark specific frames in a digital video or in the “menu mode” to navigate through hierarchical menus. The user study conducted for “jog wheel” mode showed that the SLAP knob outperforms the virtual one in terms of task completion time and accuracy. While tangible controls provide increased task performance, they are physical, and are not configurable as virtual controls. Furthermore, they reduce the interaction area on the tabletop surface and restrict user movements.

\subsubsection{Vibrotactile}
Another digital controller displayed through the surface of HapTable was tactile button. Interaction with physical buttons is an essential part of our daily routine. We use buttons daily to turn lights on, to call an elevator, to ring a doorbell, even to turn on our mobile devices. Buttons have distinct response characteristics and are easily activated by touch. However, there is limited tactile feedback available for their digital counterparts displayed on touch surfaces. To display tactile feedback for interactions with digital buttons, researchers have mainly utilized vibrotactile actuation method implemented by low-cost vibration motors and voice coils (Nashel and Razzaque, 2003; Brewster et al., 2007; Hoggan et al., 2008; Park et al., 2011)~\cite{MISSING} and more sophisticated piezo actuators (Pakkanen et al., 2010; Chen et al., 2011; Lylykangas et al., 2011; Kim et al., 2012; Kim and Tan, 2014; Wu and Smith, 2015; Ma et al., 2015, Sandia et al., 2019)~\cite{MISSING}. Park et al. (2011)~\cite{MISSING} focused on displaying tactile feedback on mobile devices when a digital button is pressed on the screen. They presented seventy-two different vibrotactile stimulus to the subjects by varying amplitude, duration, carrier signal, envelope function, and type of actuators. They suggested that, for pleasant button clicks, short rise time as well as short duration are preferable. Chen et al. (2011)~\cite{MISSING} designed and evaluated a set of simulated key clicks for key-less mobile devices equipped with piezoelectric actuators. They concluded that key clicks are perceived as “crisp” (“dull”) at the stimulation frequency of 500 Hz (125 Hz). Lylykangas et al. (2011)~\cite{MISSING} investigated the preference in type of tactile feedback displayed by piezo-actuated digital buttons under different time delays and vibration durations. Their results showed that, it is possible to create either favorable or significantly less favorable button click feedback by varying delay and duration parameters within a relatively short time window. They also concluded that the signal for tactile feedback requires careful design and control of the duration parameter. The earlier studies have mainly focused on displaying “pleasant” button click sensations using vibration cues, but not the realistic feeling. However, it is also important to relate the tactile feedback generated by vibrotactile actuators to different types of physical buttons based on measured data. Recently, Sadia et al. (2019)~\cite{MISSING}, displayed vibrotactile feedback through a touch surface to simulate the feeling of physical buttons using piezo actuators attached to it. They first recorded and analyzed the force, acceleration, and voltage data from twelve participants interacting with three different physical buttons: latch, toggle, and push buttons. Then, a button-specific vibrotactile stimulus was generated for each button by modulating the recorded accelaration signal with the resonance frequency of the surface. In their user experiments, participants were able to match the three digital buttons with their physical counterparts with a success rate of 83\%. \hl{SEUNGMOON AND VINCENT,...}

\subsubsection{Electrostatic}

In order to demonstrate that a virtual knob with frictional tactile feedback is possible on a touch surface, Emgin et al. (2019) developed a visulization table (called HapTable) including a large electrostatic display to render a tactile knob on its surface. In their approach, user rotates a virtual knob displayed through the surface using two fingers to select an item from a menu while feeling the detents of the knob and receiving frictional feedback according to their movement. The  table recognizes the “rotation” gesture of the user automatically to modulate the friction between user finger and the surface based on the electrostatic actuation method. 

\subsubsection{Ultrasonic}

Apart from the studies on vibrotactile feedback, it has been shown that a click effect, as in key press, can be created by reducing the friction as the user presses on an ultrasonically actuated touch surface (Tashiro et al., 2009; Monnoyer et al, 2016; Saleem et al., 2018). Tashiro et al. (2009)~\cite{MISSING} have rendered the feeling of buckling and restitution of mechanical buttons using Langevin-type ultrasonic transducer. They argued that the perception of button press and release are due to momentary slippage of the finger over the surface, which occurs when the friction of the surface is reduced by ultrasonic actuation. Unlike in Tashiro et al. (2009), Monnoyer et al. (2016)~\cite{MISSING} argued that the feeling of click occurs due to a sudden release of stress at the fingertip, which is accumulated when the friction of surface is high. Recently, it has been shown that there is an optimal value of finger impedance that leads to a stronger perception of haptic click effect (Monnoyer et al., 2017)~\cite{MISSING}. Moreover, the rate of change in normal force has been reported to play an important role in perception of click effect (Saleem et al., 2018)~\cite{MISSING}. \hl{FREDERIC, ULTRASONIC VIRTUAL KNOB? SOME EXAMPLES BY Hap2U?}

\hl{Giraud et al. (2013), Design and control of a haptic knob} \cite{Giraud13a}

\subsection{Tactile Rendering of Virtual Shapes and Surface Features}
\hl{CB}

\subsubsection{Vibrotactile textures}
\hl{SC}

\subsubsection{Electrovibration}
Several researchers (Meyer et al., 2013; Vardar et al., 2017; Shultz et al., 2018)~\cite{MISSING} have utilized amplitude modulation for effective rendering of tactile effects via electrovibration. Shultz et. al [36]~\cite{MISSING} observed that impedance of the gap between fingerpad and touch screen causes a volatile transition of force dynamics in the frequency range of 20-200 Hz for the case of electrovibration. They argued that amplitude modulation with a high frequency carrier voltage signal avoids this transition regime and hence, the modulated voltage signal results in a tangential force signal with a rectified DC component coming from the envelope signal and an AC component coming from the carrier signal. If the frequency of carrier signal is selected as higher than the human vibrotactile threshold level of 1 kHz [38,39]~\cite{MISSING}, then the AC component of the resulting tangential force is not perceived by the user.  In order to validate this approach experimentally, Isleyen et al. (2019)~\cite{MISSING} investigated the power spectrum of tangential forces acting on the user while he slides his finger with a constant velocity of 50 mm/s on a real square grating with a spatial period of 2.5 mm (hence, the temporal frequency is 20 Hz) under a constant normal force of 0.75 N. The power spectrum revealed a series of peaks with decreasing magnitude at frequencies that are integer multiples of the temporal frequency. As predicted by the theory, this spectrum resembled to the power spectrum of tangential forces recorded for a corresponding virtual grating rendered by low frequency square signal (envelope) at 20 Hz modulated with a high frequency sinusoidal signal (carrier) at 3 kHz more than the spectrum of the envelope signal alone.

To render textures, the researchers mostly utilized data-driven approaches. Jiao et. al [31]~\cite{MISSING} developed a data-driven algorithm for rendering virtual textures on electrostatic friction displays. They acquired force and position data while finger is sliding on 10 different fabric samples to modulate the voltage applied to the touch screen based on the estimated friction coefficients. They conducted psychophysical experiments to make a perceptual comparison between real and virtual textures and results showed that virtual textures were perceptually similar to corresponding real textures. Osguei [32]~\cite{MISSING} et. al proposed an inverse neural network model to learn from recorded real textures. They showed that the voltage signal for electrostatic actuation can be estimated by this model to render virtual textures on touch screen that resembles to the real ones. Wu et. al [34]~\cite{MISSING} proposed a rendering method for image-based textures based on the estimation of local gradients. The gradients are used to map the frequency (texture granularity) and amplitude (texture height) of the voltage signal applied to the touch screen. Their results showed that modulating frequency further improved tactile realism of virtual textures.

\hl{Seungmoon: Textures}

\hl{Data-driven textures rendered by electrovibration}

\hl{Seungmoon: Shapes}

Tactile rendering of 3D virtual shapes or bumps is possible by mapping the gradients of a surface to magnitude of friction forces (Kim et al., 2013; Osgouei et al., 2017)~\cite{MISSING}.

\hl{Vincent knows a study on shape rendering by electrovibration (Disney)}

\subsubsection{Ultrasonic textures}
\hl{Frederic: are there any papers on rendering methods? Include the closed loop in friction}


\subsection{Tactile Perception of Virtual Surface Features}
\hl{CB}

To display realistic tactile features such as textures on touch-enabled devices, it is important to understand how surface prop-erties are perceived by means of touch in the real world. Earlier studies have revealed four psychophysical dimensions related to the perception of real textures: roughness, hardness, slipperiness, and warmness [27]~\cite{MISSING}. Hollins et al. [28,29]~\cite{MISSING} have found that roughness and hardness are more robust and orthogonal to each other, while Bensmaia et al. [30]~\cite{MISSING} have shown that roughness and slipperiness are more important dimensions in differentiating textures. Hence, roughness is arguably the most important dimension in tactile perception of textures. Thus, a great deal of research has focused on discrimination and roughness perception of real textures [31]–[56]~\cite{MISSING}. The results showed significant effect of physical texture dimensions (especially, height and inter-element spacing) on tactile perception and associated neural mechanism. Temporal cues (mediated by PC-afferents) play a dominant role in the roughness perception of fine surface features (micro-textures), while spatial cues (mediated by SA1-afferents) are dominant in the roughness perception of coarser ones (macro-textures) [49,51]~\cite{MISSING}. 

On the other hand, tactile discrimination and roughness perception are less studied for virtual textures displayed on touch surfaces, and the perceptual mechanisms behind them have not been understood yet [6-8,11,14,15,57,58]~\cite{MISSING}. Since texture height, which is important for activating SA1-afferents, cannot be displayed directly by vibrating the surface in normal direction or modulating friction in tangential direction, tactile perception of virtual textures displayed on touch surfaces is expected to be different than that of the real ones.

\subsubsection{Vibrotactile}

Ahmaniemi et al. [74]~\cite{MISSING} investigated the perception of virtual textures displayed by a hand held vibrotactile actuator. They reported that the textures created with a carrier frequency of 10 Hz were per-ceived rougher than those of 20 Hz, supporting the inverted U-shaped trend observed with real textures. \hl{SEUNGMOON+VINCENT: many other studies}

\subsubsection{Electrostatic}

Vardar et al. [11]~\cite{MISSING} investigated the roughness perception of periodic gratings displayed by electrovibration. They compared four wave-forms; sine, square, triangular and saw-toothed waves with spatial period varying from 0.6 to 8 mm. The width of periodic high friction regimes (analogous to ridge width) was taken as 0.5 mm, while that of the low friction ones (analogous to groove width) was varied. The finger velocity was controlled indirectly by displaying a visual cursor moving at 50 mm/s. The results showed that square wave-form was perceived as the roughest, while there was no significant difference between the other three waveforms. The perceived roughness decreased with increasing spatial period in general, though a modest U-shaped trend was ob-served with a peak value around 2 mm. They also reported that the roughness perception of periodic gratings correlates best with the rate of change in tangential force, similar to the real gratings [47]~\cite{MISSING}. Recently, Isleyen et al. (2019, MS thesis)~\cite{MISSING} investigated the roughness perception of real gratings made of plexiglass and virtual gratings displayed by electrovibration through a touch screen for comparison. They conducted two psychophysical experiments with 10 participants to investigate the effect of spatial period and the normal force applied by finger on roughness perception of real and virtual gratings in macro size while recording the tangential forces acting on the participants' finger during the experiments. The results showed that the roughness perception of real and virtual gratings are different. They argued that this difference can be explained by the amount of fingerpad penetration into the gratings. For real gratings, penetration increased tangential forces acting on the finger, whereas for virtual ones where skin penetration is absent, tangential forces decreased with spatial period. Supporting this claim, they also found that increasing normal force increases the perceived roughness of real gratings while it causes an opposite effect for the virtual gratings. These results were consistent with the tangential force profiles recorded for both real and virtual gratings. In particular, the rate of change in tangential force (dFt/dt) as a function of spatial period and normal force followed trends similar to those obtained for the roughness estimates of real and virtual gratings, suggesting that it is a better indicator of the perceived roughness than the tangential force magnitude.

\subsubsection{Ultrasonic}

Samur et al. [20]~\cite{MISSING} have conducted discrimination experiments to evaluate the minimum detectable difference in friction using the tactile pattern display (TPad). The subjects were presented with two stimuli in sequential order and asked to identify the stimulus with higher friction. An average JND of 18\% was reported for the friction difference. This study shows the ability of humans to discriminate two surfaces based on friction, but how humans perceive a change in friction cannot be ascertained. In this regard, Messaoud et al. [22]~\cite{MISSING} have evaluated the subjects' performance in detecting a change in friction. Their results showed that the detection rate improves at lower inherent friction between finger and surface, as well as lower finger velocity of 5 mm/s compared to 20 mm/s. They also found that the detection rate is best correlated to friction contrast and a contrast greater than 0.19 is always detectable. It is shown in Saleem et al. (2017)~\cite{MISSING} that rate of change in tangential force is best correlated with the detection rate of friction change. Saleem et al. (2018)~\cite{MISSING} also showed that a step increase in friction casts a stronger perceptual effect as compared to a step fall in friction. Gueorguiev et al. [25]~\cite{MISSING} investigated the tactile perception of square pulses displayed by ultrasonic friction modulation and observed that subjects could differentiate between two pulses if the duration and transition time are extended by 2.4 and 2.1 ms, respectively. In another experiment, they found that if the duration between two pulses was shorter than 50 ms, subjects perceived them as a single pulse. In [29]~\cite{MISSING}, the authors have evaluated the threshold to detect two friction reductions of 100 ms duration, rendered 3 mm apart, using three different ultrasonically actuated surfaces made of aluminum, polypropylene and polyurethane. The rise time of vibration amplitude was controlled at 1.5 ms. The surfaces were passively scanned under the finger at 20 mm/s, while normal force was maintained at 0.7 N. They conducted threshold experiments and measured the vibration thresholds at 75\% JND as 0.17, 0.23, 0.27 um for aluminum, polypropylene and polyurethane, respectively. Furthermore, the detection rate was found to correlate well with the ratio of reduction in tangential force to pre-stimulation tangential force. The discrimination of periodic gratings, rendered on a touch surface by ultrasonic actuation was investigated in [6]~\cite{MISSING}. The surface was vibrated at a frequency of 30 kHz with an amplitude of 1.1 um. Four standard and eight comparison gratings in square waveform were rendered. The width ratio of high to low friction regimes was always kept constant. The finger velocity was not controlled. The results showed that the difference threshold (JND) increases with spatial period (0.2, 0.32, 0.47 and 0.8 mm for spatial period of 2.5, 3.5, 5 and 10 mm, respectively). Unlike real gratings [44], Weber fraction remained almost constant (varied between 8 and 10 \%). More recently, Saleem et al. (PhD thesis) investigated our ability to discriminate two consecutive changes in friction (called edges), followed by discrimination and roughness perception of multiple edges (called periodic gratings). The results showed that discrimination of two consecutive edges was significantly influenced by edge sequence: a step fall in friction (F F ) followed by a step rise in friction (RF ) was discriminated more easily than the reverse order. On the other hand, periodic gratings generated by displaying consecutive edge sequence of F F followed by RF were perceived with the same acuity as compared to vice versa. They also found that a relative difference of 14\% in spatial period was required to discriminate two periodic gratings independent of the edge sequence. Moreover, the roughness perception of periodic gratings decreased with increasing spatial period for the range that they have investigated (spatial period > 2 mm), supporting the results observed by Vardar et al. (2017)~\cite{MISSING} and Isleyen et al. (MS thesis, 2019)~\cite{MISSING} for friction modulation by electrovibration. \hl{Frederic: More?}




